The 3D kinematics of stellar substructures in the periphery of the Large Magellanic Cloud

We report the 3D kinematics of 27 Mira-like stars in the northern, eastern and southern periphery of the Large Magellanic Cloud (LMC), based on Gaia proper motions and a dedicated spectroscopic follow-up. Low-resolution spectra were obtained for more than 40 Mira-like candidates, selected to trace known substructures in the LMC periphery. Radial velocities and stellar parameters were derived for all stars. Gaia data release 3 astrometry and photometry were used to discard outliers, derive periods for those stars with available light curves, and determine their photometric chemical types. The 3D motion of the stars in the reference frame of the LMC revealed that most of the stars, in all directions, have velocities consistent with being part of the LMC disk population, out of equilibrium in the radial and vertical directions. A suite of N-body simulations was used to constrain the most likely past interaction history between the Clouds given the phase-space distribution of our targets. Model realizations in which the Small Magellanic Cloud (SMC) had three pericentric passages around the LMC best resemble the observations. The interaction history of those model realizations has a recent SMC pericentric passage ($\sim$320 Myr ago), preceded by an SMC crossing of the LMC disk at $\sim$0.97 Gyr ago, having a radial crossing distance of only $\sim$4.5 kpc. The previous disk crossing of the SMC was found to occur at $\sim$1.78 Gyr ago, with a much larger radial crossing distance of $\sim$10 kpc.

==> table1.tex <==
\begin{table*}
	\centering
	\caption{This is a caption tbc by David.}
	\label{tab:stellar_params}
\begin{tabular}{rccccccccccr}
\hline
ID    & RA        & DEC     & V$_{\rm rad}$ & $\sigma_{\rm Vrad}$ & H$_{\rm emi}$ & shift & [Fe/H]  & T$_{\rm eff}$  & logg  & [Fe/H]$_{\rm CaT}$ & Flag  \\
      & (hh:mm:ss.s) & (dd:mm:ss) & (km s$^{-1}$) & (km s$^{-1}$) & ({\AA}) & (km s$^{-1}$) & & (K) & (cm s$^{-2}$) & & \\
\hline      
BP22  & 10:10:29.0 & --31:44:53 & 320.3871 & 6.708   &            &             & --1.125 & 4091.713 & 0.684 & --1.051   & 1     \\
BP23  & 11:55:27.4 & --39:57:44 & 158.2451 & 9.548   & 6562.252   & --25.0435    & --0.913 & 3939.736 & 0.812 & --1.112   & 1     \\
BP24  & 11:17:16.7 & --36:20:11 & 324.3146 & 7.602   &            &             & --1.07  & 3834.366 & 0.0   & --1.518   & 1     \\
BP25  & 10:29:52.7 & --33:29:26 & 39.5851  & 10.688  & 6562.739   & --2.79005    & --0.986 & 4013.927 & 0.494 & --0.982   & 1     \\
BP26  & 10:39:36.2 & --37:08:53 & 109.0591 & 9.56    &            &             & --1.18  & 3747.152 & 0.0   & --0.981   & 1     \\
BP27  & 10:24:57.2 & --31:25:47 & 42.4086  & 8.326   &            &             & --0.859 & 3867.569 & 0.192 & --0.984   & 1     \\
BP28  & 10:11:16.3 & --17:41:28 & 156.8572 & 43.819  & 6563.253   & 20.7133     & --2.926 & 3500.027 & 0.138 & --3.853   & 0     \\
BP29  & 11:21:35.3 & --43:34:16 & 0.5529   & 8.649   &            &             & 0.409  & 4145.965 & 5.0   & 0.029    & 1     \\
BP30  & 10:54:28.0 & --15:59:49 & --10.0366 & 9.01    &            &             & --0.215 & 4205.23  & 4.999 & 0.5      & 1     \\
BP30  & 10:54:28.0 & --15:59:49 & --13.1262 & 8.339   &            &             & --0.126 & 4186.294 & 4.999 & 0.5      & 1     \\
BP31  & 11:49:21.1 & --16:07:42 & --3.2159  & 9.861   &            &             & --0.958 & 3919.745 & 4.792 & --1.121   & 1     \\
BP32  & 09:30:18.0 & --21:04:54 & 234.5767 & 10.699  & 6562.803   & 0.156243    & --1.302 & 4037.446 & 1.096 & --1.688   & 1     \\
BP33  & 10:07:07.0 & --19:24:04 & 313.4083 & 10.666  &            &             & --1.112 & 4039.589 & 0.378 & --1.255   & 1     \\
BP34  & 10:52:49.4 & --17:12:15 & 27.8522  & 9.645   &            &             & --0.81  & 3967.244 & 4.999 & --0.006   & 1     \\
BP35  & 11:25:38.0 & --28:55:53 & 213.7239 & 22.336  & 6562.711   & --4.06231    & 0.08   & 4491.123 & 1.28  & --2.177   & 0     \\
BP36  & 11:50:27.0 & --43:22:29 & 162.7252 & 86.679  &            &             & --1.632 & 3545.063 & 1.906 & --1.514   & 1     \\
BP37  & 12:03:52.8 & --40:37:26 & 235.8261 & 23.03   &            &             & 0.229  & 4481.466 & 0.854 & --1.911   & 0     \\
BP38  & 11:37:54.5 & --33:58:40 & 85.0656  & 12.412  &            &             & --1.012 & 3982.809 & 0.549 & --1.022   & 1     \\
BP39  & 11:45:58.0 & --27:13:38 & 160.0796 & 8.866   & 6562.464   & --15.3564    & --2.483 & 3500.021 & 0.003 & --2.676   & 1     \\
\hline
EE06  & 08:49:19.0 & --70:41:50 & 321.7739 & 7.274   &            &             & --0.964 & 3987.774 & 0.531 & --1.004   & 1     \\
EE07  & 07:43:44.4 & --69:18:05 & 314.0924 & 10.211  &            &             & --1.051 & 3833.992 & 0.242 & --1.637   & 1     \\
EE08  & 07:36:51.5 & --65:46:52 & 372.3152 & 7.772   &            &             & --0.958 & 4038.415 & 0.187 & --0.962   & 1     \\
EE09  & 06:59:30.5 & --65:27:18 & 377.313  & 7.677   &            &             & --0.961 & 3958.605 & 0.029 & --0.936   & 1     \\
EE10  & 07:33:06.8 & --73:06:27 & 318.2083 & 9.795   &            &             & --1.663 & 3595.923 & 0.011 & --1.074   & 1     \\
EE11  & 07:09:52.1 & --66:49:31 & 330.503  & 21.347  &            &             & 0.026  & 4496.491 & 1.276 & --0.011   & 1     \\
EE12  & 07:13:58.1 & --64:19:10 & 341.0652 & 7.825   &            &             & --1.113 & 4020.173 & 0.587 & --1.104   & 1     \\
EE13  & 07:22:16.5 & --63:42:15 & 295.7055 & 13.467  &            &             & 0.136  & 4499.98  & 0.8   & 0.004    & 1     \\
EE14  & 07:12:18.5 & --63:38:09 & 260.5262 & 80.619  &            &             & --2.821 & 3500.011 & 2.474 & --4.783   & 0     \\
EE15  & 07:05:00.1 & --62:06:39 & 325.7195 & 13.566  & 6562.286   & --23.4811    & --1.616 & 4066.168 & 1.616 & --1.833   & 1     \\
EE16  & 06:56:04.7 & --63:54:41 & 279.1161 & 61.278  &            &             & --2.69  & 3500.26  & 0.004 & --3.761   & 0     \\
EE17  & 08:29:56.1 & --70:29:23 & 182.2529 & 41.148  &            &             & --1.824 & 3500.131 & 1.734 & --1.35    & 1     \\
EE18  & 08:19:12.4 & --66:53:22 & 162.7932 & 10.256  &            &             & --0.703 & 4035.834 & 0.843 & --0.641   & 1     \\
EE19  & 06:41:52.5 & --62:38:53 & 312.6143 & 7.92    &            &             & --1.16  & 3895.309 & 0.401 & --1.484   & 1     \\
EE20  & 08:03:49.1 & --63:08:30 & 357.6598 & 10.255  &            &             & --0.976 & 4036.738 & 0.221 & --0.977   & 1     \\
EE21  & 07:05:05.6 & --61:45:39 & 381.9659 & 10.934  &            &             & --1.335 & 3680.007 & 0.036 & --1.751   & 1     \\
EE22  & 09:55:37.2 & --71:13:39 & 150.921  & 8.396   &            &             & --0.909 & 4083.29  & 1.304 & --0.742   & 1     \\
LA40  & 09:46:56.8 & --82:16:36 & 248.7016 & 7.782   &            &             & --1.043 & 3935.647 & 0.329 & --1.03    & 1     \\
LA41  & 08:42:51.7 & --83:30:38 & 220.5179 & 6.899   &            &             & --1.143 & 3770.162 & 0.0   & --1.041   & 1     \\
LA42  & 08:45:03.8 & --81:04:20 & 269.1006 & 7.264   & 6562.024   & --35.4671    & --1.145 & 3831.629 & 1.099 & --1.872   & 1     \\
LA43  & 10:14:40.0 & --84:36:22 & 94.7394  & 12.438  & 6562.794   & --0.267845   & --1.105 & 3959.296 & 0.751 & --1.424   & 1     \\
LA44  & 05:41:39.5 & --82:03:02 & 220.2819 & 10.705  & 6562.298   & --22.9454    & --1.192 & 3809.934 & 1.254 & --2.283   & 1     \\
\hline
MS01  & 05:57:14.3 & --53:54:02 & 302.4366 & 54.105  & 6562.812   & 0.55801     & 0.159  & 4468.771 & 1.257 & --3.22    & 0     \\
MS02  & 07:18:21.2 & --55:19:44 & 254.8999 & 53.337  &            &             & 0.463  & 4416.973 & 0.001 & --2.961   & 0     \\
MS03  & 06:48:06.4 & --53:00:33 & 328.5077 & 24.655  & 6562.708   & --4.19624    & 0.437  & 4441.196 & 0.001 & --2.522   & 0     \\
MS04  & 05:41:38.8 & --54:20:09 & 276.4727 & 13.714  & 6562.886   & 3.95071     & --1.263 & 3845.886 & 0.623 & --1.921   & 1     \\
MS04  & 05:41:38.8 & --54:20:09 & 289.2737 & 13.398  & 6562.74    & --2.72309    & --1.251 & 3851.297 & 0.529 & --2.007   & 1     \\
MS05  & 06:28:06.1 & --53:11:05 & 317.0689 & 21.15   &            &             & --0.917 & 3507.277 & 0.0   & --1.064   & 1 \\
\hline  
\end{tabular}
\end{table*}


==> table3.tex <==
\begin{table*}
	\centering
	\caption{Gaia eDR3 parallaxes and proper motions for the Mira variable candidates.}
	\label{tab:Gaia}
\begin{tabular}{rrrr}
\hline
ID    & $\omega$ & pmra           & pmdec         \\
      & (mas)    & (mas yr$^{-1}$) & (mas yr$^{-1}$) \\
\hline      
BP22  &   0.032 $\pm$ 0.020        & --0.617 $\pm$ 0.013           & --0.531 $\pm$ 0.021               \\
BP23  &   0.029 $\pm$ 0.035        & --0.572 $\pm$ 0.026           & --0.165 $\pm$ 0.030               \\
BP24  & --0.021 $\pm$ 0.025        & --0.657 $\pm$ 0.026           & --0.276 $\pm$ 0.020               \\
BP25  & --0.037 $\pm$ 0.029        & --0.324 $\pm$ 0.024           & --0.226 $\pm$ 0.027               \\
BP26  &   0.001 $\pm$ 0.022        & --0.160 $\pm$ 0.020           & --0.316 $\pm$ 0.020               \\
BP27  &   0.009 $\pm$ 0.022        & --0.329 $\pm$ 0.017           & --0.393 $\pm$ 0.022               \\
BP28  &   0.016 $\pm$ 0.022        & --0.478 $\pm$ 0.023           & --1.216 $\pm$ 0.023               \\
BP32  &   0.007 $\pm$ 0.022        & --0.265 $\pm$ 0.025           & --0.839 $\pm$ 0.015               \\
BP33  &   0.036 $\pm$ 0.021        & --0.087 $\pm$ 0.022           & --1.109 $\pm$ 0.021               \\
BP35  &   0.013 $\pm$ 0.022        & --0.898 $\pm$ 0.019           & --1.235 $\pm$ 0.016               \\
BP36  &   0.029 $\pm$ 0.028        & --1.145 $\pm$ 0.022           & --0.565 $\pm$ 0.023               \\
BP37  &   0.025 $\pm$ 0.024        & --0.717 $\pm$ 0.016           & --0.163 $\pm$ 0.015               \\
BP38  &   0.009 $\pm$ 0.025        & --0.526 $\pm$ 0.026           & --0.437 $\pm$ 0.020               \\
BP39  &   0.003 $\pm$ 0.032        & --0.592 $\pm$ 0.027           & --0.442 $\pm$ 0.020               \\
\hline                                      
EE06  & --0.023 $\pm$ 0.020        &   0.669 $\pm$ 0.025           &   2.247 $\pm$ 0.024               \\
EE07  & --0.001 $\pm$ 0.028        &   0.940 $\pm$ 0.034           &   1.344 $\pm$ 0.033               \\
EE08  & --0.016 $\pm$ 0.031        &   1.200 $\pm$ 0.041           &   1.593 $\pm$ 0.042               \\
EE09  & --0.036 $\pm$ 0.030        &   1.387 $\pm$ 0.043           &   1.244 $\pm$ 0.035               \\
EE10  &   0.007 $\pm$ 0.026        &   1.230 $\pm$ 0.033           &   1.796 $\pm$ 0.031               \\
EE11  &   0.027 $\pm$ 0.025        &   1.178 $\pm$ 0.039           &   1.381 $\pm$ 0.033               \\
EE12  &   0.021 $\pm$ 0.028        &   1.232 $\pm$ 0.036           &   1.478 $\pm$ 0.042               \\
EE13  &   0.005 $\pm$ 0.023        &   1.341 $\pm$ 0.038           &   1.366 $\pm$ 0.028               \\
EE14  & --0.017 $\pm$ 0.033        &   1.432 $\pm$ 0.073           &   1.128 $\pm$ 0.067               \\
EE15  &   0.030 $\pm$ 0.022        &   1.291 $\pm$ 0.029           &   1.134 $\pm$ 0.028               \\
EE16  & --0.018 $\pm$ 0.029        &   1.398 $\pm$ 0.030           &   1.052 $\pm$ 0.032               \\
EE17  & --0.018 $\pm$ 0.020        & --0.137 $\pm$ 0.027           &   2.147 $\pm$ 0.023               \\
EE18  & --0.010 $\pm$ 0.021        & --0.960 $\pm$ 0.028           &   1.705 $\pm$ 0.024               \\
EE19  & --0.034 $\pm$ 0.025        &   1.462 $\pm$ 0.039           &   1.218 $\pm$ 0.032               \\
EE20  &   0.011 $\pm$ 0.027        &   0.826 $\pm$ 0.035           &   1.653 $\pm$ 0.035               \\
EE21  & --0.017 $\pm$ 0.023        &   1.359 $\pm$ 0.033           &   1.201 $\pm$ 0.029               \\
EE22  &   0.034 $\pm$ 0.022        & --1.816 $\pm$ 0.027           &   2.267 $\pm$ 0.025               \\
\hline                                      
LA40  & --0.038 $\pm$ 0.024        &   0.093 $\pm$ 0.027           &   2.521 $\pm$ 0.026               \\
LA41  & --0.006 $\pm$ 0.025        &   0.873 $\pm$ 0.031           &   2.589 $\pm$ 0.030               \\
LA42  & --0.017 $\pm$ 0.026        &   0.622 $\pm$ 0.030           &   2.182 $\pm$ 0.032               \\
LA43  & --0.004 $\pm$ 0.020        & --0.232 $\pm$ 0.023           &   0.523 $\pm$ 0.022               \\
LA44  & --0.003 $\pm$ 0.024        &   2.218 $\pm$ 0.026           &   1.136 $\pm$ 0.033               \\
\hline                                      
MS01  & --0.050 $\pm$ 0.035        &   1.534 $\pm$ 0.043           &   0.083 $\pm$ 0.041               \\
MS02  & --0.023 $\pm$ 0.024        &   1.208 $\pm$ 0.029           &   0.561 $\pm$ 0.031               \\
MS03  & --0.051 $\pm$ 0.024        &   1.391 $\pm$ 0.029           &   0.476 $\pm$ 0.029               \\
MS04  & --0.018 $\pm$ 0.019        &   1.829 $\pm$ 0.023           & --0.053 $\pm$ 0.026               \\
MS05  & --0.047 $\pm$ 0.025        &   1.471 $\pm$ 0.034           &   0.384 $\pm$ 0.030               \\
\hline  
\end{tabular}
\end{table*}

